Text-Enhanced Zero-Shot Action Recognition: A training-free approach

Vision-language models (VLMs) have demonstrated remarkable performance across various visual tasks, leveraging joint learning of visual and textual representations. While these models excel in zero-shot image tasks, their application to zero-shot video action recognition (ZSVAR) remains challenging due to the dynamic and temporal nature of actions. Existing methods for ZS-VAR typically require extensive training on specific datasets, which can be resource-intensive and may introduce domain biases. In this work, we propose Text-Enhanced Action Recognition (TEAR), a simple approach to ZS-VAR that is training-free and does not require the availability of training data or extensive computational resources. Drawing inspiration from recent findings in vision and language literature, we utilize action descriptors for decomposition and contextual information to enhance zero-shot action recognition. Through experiments on UCF101, HMDB51, and Kinetics-600 datasets, we showcase the effectiveness and applicability of our proposed approach in addressing the challenges of ZS-VAR.

==> package.tex <==
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.

% If you use the hyperref package, please uncomment the following two lines
% to display URLs in blue roman font according to Springer's eBook style:
\usepackage{color}


\usepackage{pifont}
\usepackage{enumitem}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{hyperref}               % hyperlinks
\usepackage{url}                    % simple URL typesetting
\usepackage{booktabs}               % professional-quality tables
\usepackage{amsfonts}               % blackboard math symbols
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{color,colortbl}
\usepackage{nicefrac}               % compact symbols for 1/2, etc.
\usepackage{microtype}              % microtypography
\usepackage{multirow}
\usepackage{pgfplots}
\usepackage[accsupp]{axessibility}
\usepackage{multirow}
\usepackage{marginnote}
\usepackage{subcaption}
\usepackage{float}
\usepackage{caption}

\usepackage{geometry}
\usepackage{array}

\usepackage{icomma}

\usepackage{bbding}
\usepackage{leftidx}
\usepackage{bbm}
\usepackage{algorithmic}
\usepackage{textcomp}
\usepackage{siunitx}
\usepackage{tablefootnote}
\usepackage{footnote}
\usepackage{makecell}

==> table/UCF101_best_results.tex <==

\begin{table}[t]
\small
\centering
\begin{tabular}{p{3cm} p{1.5cm} p{1.5cm} }
\toprule
\textbf{Method} & Top-1(\%) & Top-5 (\%)  \\ \noalign{\vskip1.5mm}
                
\midrule
Only Label &  &    \\ \noalign{\vskip1mm}
Description &  &    \\ \noalign{\vskip1mm}
Decomposition &  &    \\ \noalign{\vskip1mm}
Context &  &    \\ \noalign{\vskip1mm}
Combination (All)    &  &  \\
\bottomrule
\end{tabular}
\caption{\textbf{Results on UCF101}}
\label{table:best_ldarl}
\end{table}


==> table/comparative_table.tex <==
\begin{table}[h]
\centering
\begin{tabular}{p{2.1cm}M{1.2cm}M{2.2cm}M{1.6cm}M{1.6cm}M{1.6cm}M{1.6cm}M{1.6cm}M{1.6cm}} % Adjust column widths
\toprule
\textbf{Method}                              & \textbf{Training}  & \textbf{Backbone} & \textbf{\# Frames} & \textbf{UCF101} & \textbf{HMDB51} & \multicolumn{2}{c}{\textbf{K600}} \\
                                    &              &             &         &    \textbf{Top1}    &   \textbf{Top1}    &   \textbf{Top1} & \textbf{Top5} \\
\midrule
\rowcolor{VisionBlue}
ER-ZSAR~\cite{chen2021elaborative}  & \checkmark & TSM         & 16    &  51.8 & 35.3  & 42.1  & 73.1 \\
\rowcolor{VisionBlue}
JigsawNet~\cite{qian2022rethinking} & \checkmark & R(2+1)D     & 16    &  56.0 & 38.7  & -     & -  \\
\rowcolor{VisionBlue}
ActionCLIP~\cite{Wang2021-fl}       & \checkmark & ViT-B/16    & 32    &  58.3 & 40.8  & 66.7  & 91.6  \\
\rowcolor{VisionBlue}
XCLIP~\cite{Ni2022-pw}              & \checkmark & ViT-B/16    & 32    &  72.0 & 44.6  & 65.2  & 86.1  \\
\rowcolor{VisionBlue}
A5~\cite{Ju2021-lz}                 & \checkmark & ViT-B/16    & 32    &  69.3 & 44.3  & 55.8  & 81.4 \\
\rowcolor{VisionBlue}
ViFi-CLIP~\cite{rasheed2022fine}    & \checkmark & ViT-B/16    & 32    &  76.8 & 51.3  & 71.2  & 92.2 \\
\rowcolor{VisionBlue}
Text4Vis~\cite{wu2023revisiting}    & \checkmark & ViT-L/14    & 16    &  -    & -     & 68.9  & -\\
\rowcolor{VisionBlue}
MAXI~\cite{lin2023match}            & \checkmark  & ViT-B/16    & 16/32 & 78.2   & 52.3 &  71.5  &  92.5     \\
\rowcolor{VisionBlue}
LSS~\cite{ranasinghe2024language}  & \checkmark  & ViT-B/16    & 8 & 74.2   & 51.4  & -  &  -     \\
CLIP~\cite{clip}                    & \ding{55}  & ViT-B/16    & 16    &  69.9  & 38.0  & 63.5 & 86.8   \\
\midrule
\rowcolor{ModelGreen}
LDAR                    & \ding{55}  & ViT-B/16    & 16    & 76.2   & 50.8 & 56.0 & 82.0 \\
\bottomrule \noalign{\vskip3mm} 
\end{tabular}
\caption{\textbf{Comparison with state-of-the-art zero-shot action recognition methods.}
We report zero-shot action recognition results on UCF101, HMDB51, and K600. We report Top1 and Top5 accuracy computed on the three official test splits. We also include the backbone used and the number of frames sampled from videos. Green is \inlineColorbox{ModelGreen}{our method}, blue highlights \inlineColorbox{VisionBlue}{training-based approaches}. 
}
\label{tab:zs_action_recog_sota}
\end{table}


==> table/hdmb51-vit16.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of Zero-Shot (ZS) Prompting Strategies on the HMDB51 Dataset Using the ViT-B/16 Model}
\label{tab:hmdb51-vitb16}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{8em}{Prompts} & \multirow{2}{5em}{Templates} & \multirow{2}{6em}{Conditioning} & \multirow{2}{6em}{Top1 Acc(\%) } & \multirow{2}{6em}{Top5 Acc(\%)}\\
 & & & & \\
\midrule
\multirow{4}{8em}{Action Class} & \tikzcmark & \tikzcmark & 48.43 & 77.12 \\
                          & \tikzcmark & \tikzxmark   & 48.69 & 77.25 \\
                          & \tikzxmark   & \tikzcmark & 42.81 & 73.59 \\
                           & \tikzxmark  & \tikzxmark  & 42.81 & 72.22 \\
\midrule
\multirow{4}{8em}{Description} & \tikzcmark & \tikzcmark & 49.48 & 78.56 \\
                               & \tikzcmark & \tikzxmark  & 50.13 & 79.15 \\
                              & \tikzxmark   & \tikzcmark & 47.06 & 78.50 \\
                               & \tikzxmark  & \tikzxmark  & 48.95 & 79.08 \\
\midrule
\multirow{4}{8em}{Decomposition}   & \tikzcmark & \tikzcmark & 49.35 & 77.84 \\
                               & \tikzcmark & \tikzxmark   & 45.56 & 73.46 \\
                               & \tikzxmark  & \tikzcmark  & 44.97 & 76.67 \\
                                & \tikzxmark  & \tikzxmark  & 41.44 & 71.18 \\
 \midrule

\multirow{4}{8em}{Context}   & \tikzcmark & \tikzcmark & 48.17 & 81.11 \\
                           & \tikzcmark & \tikzxmark   & 41.90 & 73.66 \\
                           & \tikzxmark  & \tikzcmark  & 46.27 & 76.54 \\
                           & \tikzxmark  & \tikzxmark  & 41.24 & 72.09 \\
  \midrule
\multirow{4}{8em}{All}  & \bf \tikzcmark & \bf \tikzcmark & \bf 50.78 & \bf 82.03 \\
                                    & \tikzcmark & \tikzxmark  & 48.37 & 76.99 \\
                                   & \tikzxmark  & \tikzcmark  & 49.02 & 81.24 \\
                                    & \tikzxmark  & \tikzxmark  & 44.05 & 75.56 \\
\bottomrule
\end{tabular}
\end{table}



==> table/hmdb51-vit32.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of Zero-Shot (ZS) Prompting Strategies on the HMDB51 Dataset Using the ViT-B/32 Model}
\label{tab:hmdb51-vitb32}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{8em}{Prompts} & \multirow{2}{5em}{Templates} & \multirow{2}{6em}{Conditioning} & \multirow{2}{6em}{Top1 Acc(\%) } & \multirow{2}{6em}{Top5 Acc(\%)}\\
 & & & & \\
\midrule
\multirow{4}{6em}{Action Class}    & \tikzcmark & \tikzcmark & 47.58 & 73.46 \\
                                  & \tikzcmark  & \tikzxmark  & 45.69 & 72.94 \\
                                  & \tikzxmark  & \tikzcmark  & 44.38 & 70.46 \\
                                   & \tikzxmark  & \tikzxmark  & 41.18 & 67.91 \\
 \midrule
\multirow{4}{8em}{Description}     & \tikzcmark & \tikzcmark & 45.29 & 74.18 \\
                                      & \tikzcmark & \tikzxmark   & 46.21 & 74.12 \\
                                       & \tikzxmark  & \tikzcmark & 44.25 & 72.35 \\
                                       & \tikzxmark  & \tikzxmark  & 46.80 & 75.95 \\
 \midrule
\multirow{4}{8em}{Decomposition}     & \tikzcmark & \tikzcmark & 45.95 & 74.64 \\
                                   & \tikzcmark  & \tikzxmark & 43.27 & 68.69 \\
                                 & \tikzxmark  & \tikzcmark  & 45.23 & 72.22 \\
                                   & \tikzxmark  & \tikzxmark  & 40.13 & 65.56 \\
 \midrule
\multirow{4}{8em}{Context}      & \tikzcmark & \tikzcmark & 47.19 & 76.60 \\
                              & \tikzcmark & \tikzxmark   & 43.20 & 72.03 \\
                              & \tikzxmark  & \tikzcmark  & 47.65 & 74.51 \\
                               & \tikzxmark  & \tikzxmark  & 40.46 & 70.33 \\
  \midrule
\multirow{4}{8em}{All}     & \tikzcmark & \tikzcmark & \bf 48.04 & \bf 78.50 \\
                              & \tikzcmark & \tikzxmark   & 45.75 & 74.05 \\
                              & \tikzxmark  & \tikzcmark  & 47.52 & 76.86 \\
                               & \tikzxmark  & \tikzxmark  & 43.59 & 73.86 \\
\bottomrule
\end{tabular}
\end{table}

==> table/k600-vit16.tex <==
% \documentclass{article}
% \usepackage{subcaption}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}

% \begin{document}

\begin{table}[htbp]
\centering
\caption{Comparison of Zero-Shot (ZS) Prompting Strategies on the Kinetics-600 Dataset Using the ViT-B/16 Model}
\label{tab:k600-vitb316}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{8em}{Prompts} & \multirow{2}{5em}{Templates} & \multirow{2}{6em}{Conditioning} & \multirow{2}{6em}{Top1 Acc(\%) } & \multirow{2}{6em}{Top5 Acc(\%) }\\
 & & & & \\
\midrule
\multirow{4}{8em}{Action Class}   & \tikzcmark    & \tikzcmark        & 53.89 & 79.37 \\
                                & \tikzcmark    & \tikzxmark        & 53.87 & 79.37 \\
                                & \tikzxmark    & \tikzcmark        & 53.13 & 79.79 \\
                                & \tikzxmark    & \tikzxmark        & 53.87 & 79.36 \\
\midrule
\multirow{4}{8em}{Description}  & \tikzcmark    & \tikzcmark        & 50.43 & 78.16 \\
                                & \tikzcmark    & \tikzxmark        & 51.41 & 79.03 \\
                                & \tikzxmark    & \tikzcmark        & 50.92 & 79.18 \\
                                & \tikzxmark    & \tikzxmark        & 51.37 & 79.51 \\
\midrule
\multirow{4}{8em}{Decomposition}& \tikzcmark    & \tikzcmark        & 53.76 & 80.50 \\
                                & \tikzcmark    & \tikzxmark        & 46.01 & 74.64 \\
                                & \tikzxmark    & \tikzcmark        & 53.04 & 80.11 \\
                                & \tikzxmark    & \tikzxmark        & 45.66 & 74.52 \\
\midrule
\multirow{4}{8em}{Context}      & \tikzcmark    & \tikzcmark        & 54.96 & 81.01 \\
                                & \tikzcmark    & \tikzxmark        & 45.23 & 74.79 \\
                                & \tikzxmark    & \tikzcmark        & 54.80 & 81.02 \\
                                & \tikzxmark    & \tikzxmark        & 44.46 & 74.47 \\
\midrule
\multirow{4}{8em}{All}       & \bf\tikzcmark & \bf \tikzcmark  &\bf 55.76 & \bf 81.98 \\
                                & \tikzcmark    & \tikzxmark        & 49.37 & 77.89 \\
                                & \tikzxmark    & \tikzcmark        & 55.96 & 81.99\\
                                & \tikzxmark    & \tikzxmark        & 49.59 & 78.10 \\

\bottomrule
\end{tabular}
\end{table}

% \end{document}

==> table/k600-vit32.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of Zero-Shot (ZS) Prompting Strategies on the Kinetics-600 Dataset Using the ViT-B/32 Model}
\label{tab:k600-vitb32}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{8em}{Prompts}   & \multirow{2}{5em}{Templates} & \multirow{2}{6em}{Conditioning} & \multirow{2}{6em}{Top1 Acc(\%) } & \multirow{2}{6em}{Top5 Acc(\%) }\\
 & & & & \\
\midrule
\multirow{4}{8em}{Action Class}       & \tikzcmark    & \tikzcmark    & 47.96 & 75.30 \\
                                    & \tikzcmark    & \tikzxmark    & 48.12 & 75.37 \\
                                    & \tikzxmark    & \tikzcmark    & 48.84 & 75.35 \\
                                    & \tikzxmark    & \tikzxmark    & 47.61 & 74.77 \\
                                    \midrule
\multirow{4}{8em}{Description}      & \tikzcmark    & \tikzcmark    & 47.16 & 74.99 \\
                                    & \tikzcmark    & \tikzxmark    & 47.46 & 75.38 \\
                                    & \tikzxmark    & \tikzcmark    & 46.65 & 74.52 \\
                                    & \tikzxmark    & \tikzxmark    & 47.23 & 74.68 \\
                                \midrule
\multirow{4}{8em}{Decomposition}    & \tikzcmark    & \tikzcmark    & 48.49 & 76.37 \\
                                    & \tikzcmark    & \tikzxmark    & 42.13 & 70.26 \\
                                    & \tikzxmark    & \tikzcmark    & 48.32 & 75.77 \\
                                    & \tikzxmark    & \tikzxmark    & 40.79 & 69.19 \\
                                \midrule
\multirow{4}{8em}{Context}          & \tikzcmark    & \tikzcmark    & 49.67 & 77.21 \\
                                    & \tikzcmark    & \tikzxmark    & 40.83 & 70.20 \\
                                    & \tikzxmark    & \tikzcmark    & 49.33 & 76.72 \\
                                    & \tikzxmark    & \tikzxmark    & 38.51 & 67.32 \\
                                \midrule
\multirow{4}{8em}{All}         & \bf\tikzcmark & \bf\tikzcmark & \bf 50.82 & \bf 78.36 \\
                                    & \tikzcmark    & \tikzxmark    & 44.89 & 73.26 \\
                                    & \tikzxmark    & \tikzcmark    & 51.05 & 78.00 \\
                                    & \tikzxmark    & \tikzxmark    & 43.87 & 72.54 \\
\bottomrule
\end{tabular}
\end{table}



==> table/method_table_vit16_vit_32_2_column.tex <==
\begin{table}[h]
\centering
\begin{subtable}[b]{0.5\linewidth}
    \centering
        \begin{tabular}{lc}
            \toprule
                \textbf{Method} & Top-1/Top-5 (\%) \\ \noalign{\vskip0.5mm}
                \midrule
                % \multirow{2}{4em}{Average}  & Top-1 49.42  $\pm$ 1.04\\
                %  & Top-5 79.48 $\pm$ 1.84 \\
                % \midrule\midrule
                Action Class             & 48.69/77.25   \\ \noalign{\vskip1mm} %FALSE-TRUE
                Description             & 50.13/79.15   \\ \noalign{\vskip1mm} %FALSE-TRUE
                Decomposition           & 49.35/77.84   \\ \noalign{\vskip1mm} %TT
                Context                 & 48.17/81.11   \\ \noalign{\vskip1mm} %TT
               {\cellcolor[HTML]{9DE614}}  Combination   & {\cellcolor[HTML]{9DE614}}  50.78/82.03   \\
            \bottomrule
        \end{tabular}
    \caption{HMDB51 ViT-B/16}
\end{subtable}%
\begin{subtable}[b]{0.5\linewidth}
    \centering
        \begin{tabular}{lc}
            \toprule
                \textbf{Method} & Top-1/Top-5 (\%) \\ \noalign{\vskip0.5mm}
                \midrule
                % \multirow{2}{4em}{Average}  & Top-1 74.24  $\pm$ 1.13\\
                %  & Top-5 95.56 $\pm$ 0.92 \\
                % \midrule\midrule
                Action Class        &  72.94/94.21    \\ \noalign{\vskip1mm} %FT
                Description        &  73.33/96.51    \\ \noalign{\vskip1mm} %FT
                Decomposition      &  74.70/95.40    \\ \noalign{\vskip1mm} %TT
                Context            &  74.33/95.40    \\ \noalign{\vskip1mm} %TT
                {\cellcolor[HTML]{9DE614}} Combination&  {\cellcolor[HTML]{9DE614}} 76.16/96.27     \\ 
\bottomrule
\end{tabular}
        \caption{UFC101 ViT-B/16}
    \end{subtable}
\begin{subtable}[b]{0.5\linewidth}
    \centering
        \begin{tabular}{lc}
            \toprule
                \textbf{Method} & Top-1/Top-5 (\%) \\ \noalign{\vskip0.5mm}
                \midrule
                % \multirow{2}{4em}{Average}  & Top-1 54.00  $\pm$ 1.55\\
                %  & Top-5 80.58 $\pm$ 1.10 \\
                % \midrule\midrule
Action Class             & 53.89/79.37     \\ \noalign{\vskip1mm} %TT
Description             & 51.41/79.03     \\ \noalign{\vskip1mm} %FT
Decomposition           & 53.76/80.50     \\ \noalign{\vskip1mm} %TT
Context                 & 54.96/81.01     \\ \noalign{\vskip1mm} %TT
{\cellcolor[HTML]{9DE614}} Combination    & {\cellcolor[HTML]{9DE614}} 55.96/81.99     \\ \noalign{\vskip1mm} %FT
\bottomrule
\end{tabular}
        \caption{Kinetics-600 ViT-B/16}
    \end{subtable}
    \caption{XXXXX ViT-B/16 }
\end{table}









\begin{table}[h]
\centering
\begin{subtable}[b]{0.5\linewidth}
    \centering
        \begin{tabular}{lc}
            \toprule
                \textbf{Method} & Top-1/Top-5 (\%) \\ \noalign{\vskip0.5mm}
                \midrule
                % \multirow{2}{4em}{Average}  & Top-1 47.11  $\pm$ 0.71 \\
                %  & Top-5 75.83 $\pm$ 1.71 \\
                % \midrule\midrule
                Action Class             &  47.58/73.46   \\ \noalign{\vskip1mm} %TT
                Description             &   46.80/75.95  \\ \noalign{\vskip1mm} %FFF
                Decomposition           &   45.95/74.64  \\ \noalign{\vskip1mm} %TT
                Context                 &   47.19/76.60  \\ \noalign{\vskip1mm} %TT
               {\cellcolor[HTML]{9DE614}}  Combination   & {\cellcolor[HTML]{9DE614}} 48.04/78.50     \\
            \bottomrule
        \end{tabular}
    \caption{HMDB51 ViT-B/32}
\end{subtable}%
\begin{subtable}[b]{0.5\linewidth}
    \centering
        \begin{tabular}{lc}
            \toprule
                \textbf{Method} & Top-1/Top-5 (\%) \\ \noalign{\vskip0.5mm}
                \midrule
                % \multirow{2}{4em}{Average}  & Top-1  70.73  $\pm$ 1.21 \\
                %  & Top-5 93.34  $\pm$ 1.07   \\
                % \midrule\midrule
                Action Class        &    69.15/91.86  \\ \noalign{\vskip1mm} %TT
                Description        & 69.81/94.58   \\ \noalign{\vskip1mm} %TF
                Decomposition      &  70.61/92.60     \\ \noalign{\vskip1mm} %TT
                Context            & 71.53/93.15      \\ \noalign{\vskip1mm} %TT
                {\cellcolor[HTML]{9DE614}} Combination&  {\cellcolor[HTML]{9DE614}} 72.56/94.55      \\ 
\bottomrule
\end{tabular}
        \caption{UFC101 ViT-B/16}
    \end{subtable}
\begin{subtable}[b]{0.5\linewidth}
    \centering
        \begin{tabular}{lc}
            \toprule
                \textbf{Method} & Top-1/Top-5 (\%) \\ \noalign{\vskip0.5mm}
                \midrule
                % \multirow{2}{4em}{Average}  & Top-1    $\pm$  \\
                %  & Top-5   $\pm$   \\
                % \midrule\midrule
Action Class            &   69.15/91.86    \\ \noalign{\vskip1mm} %TT
Description             &   69.81/94.58    \\ \noalign{\vskip1mm} %FT
Decomposition           &   71.53/93.15    \\ \noalign{\vskip1mm} %TT
Context                 &   72.56/94.55    \\ \noalign{\vskip1mm} %TT
{\cellcolor[HTML]{9DE614}} Combination    & {\cellcolor[HTML]{9DE614}}      \\ \noalign{\vskip1mm} %FT
\bottomrule
\end{tabular}
        \caption{Kinetics-600 ViT-B/32}
    \end{subtable}
    \caption{XXXXX ViT-B/32 }
\end{table}

==> table/ucf101-vit32.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of Zero-Shot (ZS) Prompting Strategies on the UCF101 Dataset Using the ViT-B/32 Model}
\label{tab:ucf101-vitb32}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{8em}{Prompts} & \multirow{2}{5em}{Templates} & \multirow{2}{6em}{Conditioning} & \multirow{2}{6em}{Top1 Acc(\%) } & \multirow{2}{6em}{Top5 Acc(\%)}\\
 & & & & \\
\midrule
\multirow{4}{8em}{Action Class}  & \tikzcmark & \tikzcmark & 69.15\% & 91.86\% \\
    & \tikzcmark &  \tikzxmark & 68.86\% & 91.81\%  \\
  & \tikzxmark   & \tikzcmark & 68.44\% & 90.64\%  \\
   & \tikzxmark  & \tikzxmark  & 67.70\% & 90.77\% \\
\midrule

\multirow{4}{8em}{Description}  & \tikzcmark & \tikzcmark & 69.57\% & 94.37\%  \\
  & \tikzcmark  & \tikzxmark  & 69.81\% & 94.58\% \\
  & \tikzxmark  & \tikzcmark  & 66.93\% & 93.05\% \\
   & \tikzxmark  & \tikzxmark  & 70.71\% & 94.21\% \\
 \midrule
\multirow{4}{8em}{Decomposition}   & \tikzcmark & \tikzcmark & 70.61\% & 92.60\% \\
    & \tikzcmark & \tikzxmark  & 61.54\% & 87.95\% \\
    & \tikzxmark  & \tikzcmark & 70.16\% & 92.60\% \\
    & \tikzxmark  & \tikzxmark  & 59.87\% & 86.12\% \\
\midrule
\multirow{4}{8em}{Context}   & \tikzcmark & \tikzcmark & 71.53\% & 93.15\% \\
    & \tikzcmark & \tikzxmark   & 63.68\% & 91.28\% \\
   & \tikzxmark  & \tikzcmark  & 70.76\% & 92.92\% \\
    & \tikzxmark  & \tikzxmark  & 62.33\% & 91.28\% \\
\midrule
\multirow{4}{8em}{All}   & \bf \tikzcmark & \bf \tikzcmark & \bf 72.56\% & \bf 94.55\% \\
   & \tikzcmark & \tikzxmark   & 68.73\% & 92.81\% \\
   & \tikzxmark  & \tikzcmark  & 72.16\% & 94.03\% \\
    & \tikzxmark  & \tikzxmark  & 68.91\% & 93.05\% \\
\bottomrule
\end{tabular}
\end{table}


==> table/ufc101-vit16.tex <==
\begin{table}[h!]
\centering
\caption{Comparison of Zero-Shot (ZS) Prompting Strategies on the UCF101 Dataset Using the ViT-B/16 Model}
\label{tab:ucf101-vitb16}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{8em}{Prompts} & \multirow{2}{5em}{Templates} & \multirow{2}{6em}{Conditioning} & \multirow{2}{6em}{Top1 Acc(\%) } & \multirow{2}{6em}{Top5 Acc(\%)}\\
 & & & & \\
\midrule
\multirow{4}{8em}{Action Class} & \tikzcmark & \tikzcmark & 72.06 & 94.16 \\
   & \tikzcmark & \tikzxmark  & 72.77 & 94.21 \\
   & \tikzxmark   & \tikzcmark & 71.90 & 93.63 \\
   & \tikzxmark  & \tikzxmark  & 72.88 & 93.68 \\
\midrule
\multirow{4}{8em}{Description} & \tikzcmark & \tikzcmark & 73.33 & 96.51 \\
   & \tikzcmark  & \tikzxmark & 73.38 & 95.98 \\
   & \tikzxmark  & \tikzcmark & 67.80 & 93.84 \\
   & \tikzxmark  & \tikzxmark  & 71.69 & 95.32 \\
\midrule
\multirow{4}{8em}{Decomposition} & \tikzcmark & \tikzcmark & 74.70 & 94.53 \\
   & \tikzcmark & \tikzxmark   & 65.05 & 89.96 \\
   & \tikzxmark  & \tikzcmark  & 74.41 & 94.34 \\
   & \tikzxmark  & \tikzxmark  & 62.81 & 89.27 \\
\midrule
\multirow{4}{8em}{Context} & \tikzcmark & \tikzcmark & 74.33 & 95.40 \\
   & \tikzcmark & \tikzxmark   & 67.54 & 93.42 \\
   & \tikzxmark  & \tikzcmark  & 73.59 & 95.22 \\
    & \tikzxmark  & \tikzxmark  & 64.76 & 92.68 \\
\midrule
\multirow{4}{8em}{All} & \bf \tikzcmark & \bf \tikzcmark & \bf 76.16 & \bf 96.27 \\
   & \tikzcmark & \tikzxmark   & 72.56 & 94.61 \\
    & \tikzxmark  & \tikzcmark & 75.81 & 95.88 \\
    & \tikzxmark  & \tikzxmark  & 70.10 & 94.00 \\

\bottomrule
\end{tabular}
\end{table}

==> table/zsar_tab.tex <==
\begin{table*}[!tb]%[!htbp]
\scriptsize
\centering
% \begin{tabular}{@{}c M{0.8cm} M{0.8cm} M{0.8cm} M{0.7cm} M{0.7cm}M{0.7cm}@{}}
% \begin{tabular}{@{}l @{\hspace{2em}}cccccccccccccc}
\begin{tabular}{cccc}
\toprule
Model & UCF101 & HMDB51 & K600 \\
\midrule
\multicolumn{2}{l}{CLIP~\cite{clip}} & 69.93 / 92.7 & 38.02 / 66.34 & 63.48 / 86.80 \\
\midrule
\multicolumn{2}{l}{\OurMethod}  & 69.93 / 92.7 & 38.02 / 66.34 & 63.48 / 86.80 \\
\midrule
\multicolumn{2}{l}{\OurMethod} & 69.93 / 92.7 & 38.02 / 66.34 & 63.48 / 86.80 \\

% K400 & 400 & \textbf{78.18} / \textbf{96.03} & \textbf{50.35} / \textbf{77.10} &  \textbf{70.78} / \textbf{92.17} & \textbf{5.74} / \textbf{17.70} & \textbf{23.89} & \textbf{3.06} / \textbf{9.46} & \textbf{22.41} / \textbf{45.83} \\
% MiniKinetics & 200 & 75.10 / 95.82 & \underline{48.34} / \underline{76.95} & \underline{69.23} / 90.92 & \textbf{6.50} / \textbf{18.76} & \underline{22.70} & \underline{2.40} / \underline{8.04} & \textbf{22.50} / \textbf{46.01} \\
% K400+WebVid2.5M & 800 & 75.99 / 96.00 & \underline{45.97} / 73.94 & 69.14 / \underline{91.13} & \underline{4.81} / \underline{15.79} & 22.67 & 2.11 / \underline{8.00} & 20.92 / 43.99 \\
% K400+WebVid2.5M & 1200 & 75.72 / \underline{96.02}  & 45.51 / \underline{73.97} & \underline{69.36} / 91.11 & 4.21 / 15.15 & 22.35 & \underline{2.39} / 7.98 & \underline{21.29} / \underline{44.33}  \\
% K400+WebVid2.5M & 1600 & \underline{76.14} / 96.01 & 44.84 / 71.79 & 69.23 / 91.10 & 4.42 / 14.71 & \underline{22.89} & 2.14 / 7.71 & 20.69 / 43.59 \\
% UCF101 & 101 & -  \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Language Driven Zero-shot Action Recognition  Too-1 and top-5}

\label{tab:zsar}
% \label{tab:yti_state_of_the_art}
\end{table*}
